Higher-order Context-free Session Types in System F

We present an extension of System F with higher-order context-free session types. The mixture of functional types with session types has proven to be a challenge for type equivalence formalization: whereas functional type equivalence is often rule-based, session type equivalence usually follows a semantic approach based on bisimulations. We propose a unifying approach that handles the equivalence of functional and session types together. We present three notions of type equivalence: a syntactic rule-based version, a semantic bisimulation-based version, and an algorithmic version by reduction to the problem of bisimulation of simple grammars. We prove that the three notions coincide and derive a decidability result for the type equivalence problem of higher-order context-free session types.

==> eptcsdata.tex <==
\providecommand{\firstpage}{24}
\providecommand{\publicationstatus}{M. Carbone and R. Neykova (Eds.): 13th International\\
Workshop on Programming Language Approaches to\\
Concurrency and Communication-cEntric Software\\
EPTCS 356, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.356.3}{10.4204/EPTCS.356.3}}

